PartGLEE: A Foundation Model for Recognizing and Parsing Any Objects

We present PartGLEE, a part-level foundation model for locating and identifying both objects and parts in images. Through a unified framework, PartGLEE accomplishes detection, segmentation, and grounding of instances at any granularity in the open world scenario. Specifically, we propose a Q-Former to construct the hierarchical relationship between objects and parts, parsing every object into corresponding semantic parts. By incorporating a large amount of object-level data, the hierarchical relationships can be extended, enabling PartGLEE to recognize a rich variety of parts. We conduct comprehensive studies to validate the effectiveness of our method, PartGLEE achieves the state-of-the-art performance across various part-level tasks and obtain competitive results on object-level tasks. The proposed PartGLEE significantly enhances hierarchical modeling capabilities and part-level perception over our previous GLEE model. Further analysis indicates that the hierarchical cognitive ability of PartGLEE is able to facilitate a detailed comprehension in images for mLLMs. The model and code will be released at https://provencestar.github.io/PartGLEE-Vision/ .

==> table/part_datasets_categories.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\caption{All categories in part-level datasets with hierarchical correspondences.}
\begin{center}
\vspace{-2em}
\resizebox{0.87\columnwidth}{!}{
\begin{tabular}{c r l l l}
% \begin{tabular}{p{2.5cm}p{4cm}{\centering\arraybackslash}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}p{2cm}}
\toprule
Dataset Name & Id & Type & Object Categories &  Part Categories\\
\midrule
% ---------------------------
\multirow{20}{*}{Pascal Part\cite{chen2014detect}}
& 1 & Base & aeroplane & body, wing, tail, wheel \\
% ---------------
& 2 & Base & bicycle & wheel, handlebar, saddle \\
% ---------------
& 3 & Base & bird & beak, head, eye, foot, leg, wing, neck, tail, torso \\
% ---------------
& 4 & Base & boat & - \\
% ---------------
& 5 & Base & bottle & body, cap \\
% ---------------
& 6 & Novel & bus & license plate, door, headlight, mirror, window, wheel\\
% ---------------
& 7 & Base & car & license plate, door, headlight, mirror, window, wheel\\
% ---------------
& 8 & Base & cat & head, leg, paw, ear, eye, neck, nose, tail, torso \\
% ---------------
& 9 & - & chair & - \\
% ---------------
& 10 & Base & cow & head, leg, ear, eye, horn, muzzle, neck, tail, torso\\
% ---------------
& 11 & - & diningtable & -\\
% ---------------
& 12 & Novel & dog & head, leg, paw, ear, eye, muzzle, neck, nose, tail, torso \\
% ---------------
& 13 & Base & horse & head, leg, ear, eye, muzzle, neck, tail, torso \\
% ---------------
& 14 & Base & motorbike & wheel, handlebar, headlight, saddle \\ 
% ---------------
& 15 & Base & person & hair, head, ear, eye, nose, neck, mouth, arm, hand, leg, foot, torso \\
% ---------------
& 16 & Base &  pottedplant & plant, pot\\
% ---------------
& 17 & Base & sheep & head, leg, ear, eye, horn, muzzle, neck, tail, torso \\
% ---------------
& 18 & - & sofa & -\\
% ---------------
& 19 & - & train & -\\
% ---------------
& 20 & - & tvmonitor & -\\
\noalign{\smallskip} \hline \noalign{\smallskip}
% ---------------------------
\multirow{11}{*}{PartImageNet\cite{he2021partimagenet}}
& 1 & - & Quadruped & head, body, foot, tail \\
% ---------------
& 2 & - & Biped & head, body, hand, foot, tail \\
% ---------------
& 3 & - & Fish & head, body, fin, tail\\
% ---------------
& 4 & - & Bird & head, body, wing, foot, tail \\
% ---------------
& 5 & - & Snake & head, body \\
% ---------------
& 6 & - & Reptile & head, body, foot, tail\\
% ---------------
& 7 & - & Car & body, tier, side mirror \\
% ---------------
& 8 & - & Bicycle & head, body, seat, tier \\
% ---------------
& 9 & - & Boat & body, sail \\
% ---------------
& 10 & - & Aeroplane & head, body, wing, engine, tail \\
% ---------------
& 11 & - & Bottle & body, mouth\\
\noalign{\smallskip} \hline \noalign{\smallskip}
% ---------------------------
\multirow{20}{*}{Pascal-Part-116\cite{wei2023ov}}
& 1 & Base & aeroplane & body, stern, wing, tail, engine, wheel \\
% ---------------
& 2 & Base & bicycle & wheel, saddle, handlebar, chainwheel, headlight \\
% ---------------
& 3 & Novel & bird & wing, tail, head, eye, beak, torso, neck, leg, foot \\
% ---------------
& 4 & Base & boat & - \\
% ---------------
& 5 & Base & bottle & body, cap \\
% ---------------
& 6 & Base & bus & wheel, headlight, front, side, back, roof,
mirror, license plate, door, window\\
% ---------------
& 7 & Novel & car & wheel, headlight, front, side, back, roof,
mirror, license plate, door, window]\\
% ---------------
& 8 & Base & cat & tail, head, eye, torso, neck, leg, nose, paw, ear \\
% ---------------
& 9 & - & chair & - \\
% ---------------
& 10 & Base & cow & tail, head, eye, torso, neck, leg, ear, muzzle, horn\\
% ---------------
& 11 & - & diningtable & -\\
% ---------------
& 12 & Novel & dog & tail, head, eye, torso, neck, leg, nose,
paw, ear, muzzle \\
% ---------------
& 13 & Base & horse & tail, head, eye, torso, neck, leg, ear, muzzle, hoof \\
% ---------------
& 14 & Novel & motorbike & wheel, saddle, handlebar, headligh \\ 
% ---------------
& 15 & Base & person & head, eye, torso, neck,
leg, foot, nose, ear, eyebrow, mouth, hair, lower arm, upper arm, hand \\
% ---------------
& 16 & Base & pottedplant & pot, plant\\
% ---------------
& 17 & Novel & sheep & tail, head, eye, torso, neck, leg, ear, muzzle, horn] \\
% ---------------
& 18 & - & sofa & -\\
% ---------------
& 19 & Base & train & headlight, head, front, side, back, roof, coach\\
% ---------------
& 20 & Base & tvmonitor & screen\\
\noalign{\smallskip} \hline \noalign{\smallskip}
% ---------------------------
\multirow{44}{*}{ADE-Part-234\cite{wei2023ov}}
& 1 & Base & person & arm, back, foot, gaze, hand, head, leg, neck, torso \\
& 2 & Base & door & door frame, handle, knob, panel \\
& 3 & Base & clock & face, frame \\
& 4 & Base & toilet & bowl, cistern, lid \\
& 5 & Base & cabinet & door, drawer, front, shelf, side, skirt, top \\
& 6 & Base & sink & bowl, faucet, pedestal, tap, top \\
& 7 & Base & lamp & arm, base, canopy, column, cord, highlight,light source, shade,tube \\
& 8 & Base & sconce & arm, backplate, highlight, light source, shade \\
& 9 & Base & chair & apron, arm, back, base, leg, seat, seat cushion, skirt, stretcher \\
& 10 & Base & chest of drawers & apron, door, drawer, front, leg \\
% ---------------
& 11 & Base & chandelier & arm, bulb, canopy, chain, cord, highlight, light source, shade \\
& 12 & Base & bed & footboard, headboard, leg, side rail \\
& 13 & Base & table & apron, drawer, leg, shelf, top, wheel\\
& 14 & Base & armchair & apron, arm, back, back pillow, leg, seat, seat base, seat cushion \\
& 15 & Novel & ottoman & back, leg, seat \\
& 16 & Base & shelf & door, drawer, front, shelf \\
& 17 & Novel & swivel chair & back, base, seat, wheel \\
& 18 & Novel & fan & blade, canopy, tube \\
& 19 & Base & coffee table & leg, top\\
& 20 & Novel & stool & leg, seat \\
& 21 & Base & sofa & arm, back, back pillow, leg, seat base, seat cushion, skirt  \\
% ---------------
& 22 & Base & computer & computer case, keyboard, monitor, mouse \\
& 23 & Novel & desk & apron, door, drawer, leg, shelf, top \\
& 24 & Base & wardrobe & door, drawer, front, leg, mirror, top \\
& 25 & Base & car & bumper, door, headlight, hood, license plate, logo, mirror, wheel, window, wiper \\
& 26 & Novel & bus & bumper, door, headlight, license plate, logo, mirror, wheel, window, wiper \\
& 27 & Novel & oven & button panel, door, drawer, top \\
& 28 & Base & cooking stove & burner, button panel, door, drawer, oven, stove\\
& 29 & Base & microwave & button panel, door, front, side, top, window \\
& 30 & Base & refrigerator & button panel, door, drawer, side \\
& 31 & Novel & kitchen island & door, drawer, front, side, top \\
% ---------------
& 32 & Base & dishwasher & button panel, handle, skirt \\
& 33 & Base & bookcase & door, drawer, front, side\\
& 34 & Base & television receiver & base, buttons, frame, keys, screen, speaker \\
& 35 & Base & glass & base, bowl, opening, stem \\
& 36 & Base & pool table & bed, leg, pocket \\
& 37 & Novel & van & bumper, door, headlight, license plate, logo, mirror, taillight, wheel, window, wiper \\
& 38 & Base & airplane & door, fuselage, landing gear, propeller, stabilizer, turbine engine, wing \\
& 39 & Novel & truck & bumper, door, headlight, license plate, logo, mirror, wheel, windshield\\
& 40 & Novel & minibike & license plate, mirror, seat, wheel \\
& 41 & Base & washer & button panel, door, front, side \\
& 42 & Novel & bench & arm, back, leg, seat \\
% ---------------
& 43 & Base & traffic light & housing, pole \\
& 44 & Base & light & aperture, canopy, diffusor, highlight, light source, shade \\
\bottomrule
\end{tabular}}
\end{center}
\label{table:part_datasets_categories}
\vspace{-2em}
\end{table}
\setlength{\tabcolsep}{1.4pt}
